Monoidal Width: Capturing Rank Width

Monoidal width was recently introduced by the authors as a measure of the complexity of decomposing morphisms in monoidal categories. We have shown that in a monoidal category of cospans of graphs, monoidal width and its variants can be used to capture tree width, path width and branch width. In this paper we study monoidal width in a category of matrices, and in an extension to a different monoidal category of open graphs, where the connectivity information is handled with matrix algebra and graphs are composed along edges instead of vertices. We show that here monoidal width captures rank width: a measure of graph complexity that has received much attention in recent years.

==> eptcsdata.tex <==
\providecommand{\firstpage}{268}
\providecommand{\publicationstatus}{J. Master \& M. Lewis (Eds.): Fifth International\\
Conference on Applied Category Theory (ACT 2022).\\
EPTCS 380, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.380.16}{10.4204/EPTCS.380.16}}

